Deep Configuration Performance Learning: A Systematic Survey and Taxonomy

Performance is arguably the most crucial attribute that reflects the quality of a configurable software system. However, given the increasing scale and complexity of modern software, modeling and predicting how various configurations can impact performance becomes one of the major challenges in software maintenance. As such, performance is often modeled without having a thorough knowledge of the software system, but relying mainly on data, which fits precisely with the purpose of deep learning. In this paper, we conduct a comprehensive review exclusively on the topic of deep learning for performance learning of configurable software, covering 1,206 searched papers spanning six indexing services, based on which 99 primary papers were extracted and analyzed. Our results outline key statistics, taxonomy, strengths, weaknesses, and optimal usage scenarios for techniques related to the preparation of configuration data, the construction of deep learning performance models, the evaluation of these models, and their utilization in various software configuration-related tasks.We also identify the good practices and potentially problematic phenomena from the studies surveyed, together with a comprehensive summary of actionable suggestions and insights into future opportunities within the field. To promote open science, all the raw results of this survey can be accessed at our repository: https://github.com/ideas-labo/DCPL-SLR.

==> discussion.tex <==
\section{Discussion: The Common Practice of Current Work}
\label{sec:discussion}
This section provides an in-depth discussion of the common practice identified from the results of the existing work. Through this, we aim to summarize the good behaviors that all of us can follow and alarm the ``bad smell'' that should be better dealt with in future work of configuration performance learning. Specifically, we discuss the common practice observed with respect to different themes of the research questions, namely \textit{Preparation}, \textit{Modeling}, \textit{Evaluation}, and \textit{Application}.



%\subsection{The Common Practice of Current Work}

%

\subsection{Preparation} 

%Table~\ref{tb:preprocessing} provides a comprehensive summary of the preprocessing techniques employed in the surveyed studies, revealing several noteworthy trends. 

Drawing on the results from Section~\ref{sec:rq1}, we observe various phenomena related to different phases within the preparation stage of deep configuration performance learning. Specifically, there are several good practices:
\begin{itemize}
%it is recognized that software configurations often exist in various scales and units, making it difficult to learn the common representations between the features, and researchers have applied normalization techniques to bridge this gap; secondly,
    \item Configuration performance data often exhibits some characteristics that are difficult to learn by deep learning models, and addressing these challenges can lead to improved model performance, which puts high demands on data preprocessing to improve the data quality. Therefore, it is a good practice that a variety of characteristics have been tackled in the primary studies. For example, the configuration space of software is demonstrated to be high-dimensional and sparse, which has been mitigated by regularization and dimension extraction techniques; and the primary studies also reveal that raw performance datasets often have outliers, imbalance, and multicollinearity issues. By addressing these issues, these studies have enhanced the effectiveness and efficiency of performance models and provided insights for future studies.
    \item Encouragingly, it has been demonstrated that the choice of encoding scheme is critical since it profoundly impacts the prediction accuracy and time consumption of deep learning models~\cite{DBLP:conf/msr/GongC22}. For instance, one-hot encoding tends to yield the highest accuracy albeit with longer training times compared to other schemes, while label encoding often leads to faster training times. Thereby, they provide practical rules for choosing the best encoding scheme and enable future researchers to make more informative decisions.
    \item The configuration space can be enormous, while the resources available for collecting training samples are often limited. Therefore, it is crucial to carefully select the most appropriate configurations to train performance models. However, one of the challenges lies in determining the criteria for sample selection. In the current literature, a good practice is that a few studies have addressed this issue by employing heuristic sampling methods tailored to specific requirements. Especially,~\citet{wang2021morphling} leverage SMBO to guide the sampling process with a surrogate Gaussian Process model to minimize the uncertainty of the samples in each iteration. By combining with various surrogate models, SMBO can potentially yield diverse sampling results, providing potential for future studies to investigate.
\end{itemize}

On the other hand, the bad smells we observed are as follows:
\begin{itemize}
    \item It is observed that a majority of the primary studies (44 out of 85) have paid inadequate attention to the importance of preprocessing methods. Neglecting these crucial steps can severely limit the performance and effectiveness of deep learning models~\cite{DBLP:journals/jss/PereiraAMJBV21}. Therefore, it is imperative for future studies to recognize the significance of preprocessing techniques and incorporate them systematically to ensure optimal model performance.
    \item The influence of encoding schemes is underestimated by a majority of the studies, which solely rely on an ad-hoc way without providing justifications for the encoding schemes. This oversight can be detrimental, as it leaves other researchers unclear of which encoding schemes is suitable, potentially resulting in ambiguous data formats for deep learning tasks~\cite{DBLP:journals/jmlr/AlayaBGG19, DBLP:conf/kbse/BaoLWF19}.
    \item Despite the availability of various sampling strategies, a significant portion of the studies tends to focus on the most straightforward approach, namely random sampling. While random sampling is effective in representing the distribution of the dataset, it can lead to overfitting in highly sparse systems, as many of the features may prove ineffective for software performance analysis~\cite{DBLP:conf/wosp/PereiraA0J20}. This can be even more problematic considering the fact that there exist invalid configurations~\cite{DBLP:conf/kbse/JamshidiSVKPA17}. Therefore, researchers need to explore alternative sampling methods in such scenarios to enhance the accuracy of the performance models.
\end{itemize}




\subsection{Modeling} 


Recall from Section~\ref{sec:rq2}, the modeling stage is also a major stage in deep configuration performance learning for which we confirm several common practices. In particular, our analysis reveals the following positive practices:
\begin{itemize}
    \item Encouragingly, a majority of studies recognize the significance of addressing sparsity and overfitting, which are critical for causing the degradation of predictive models, urging the application of a diverse range of handling techniques~\cite{DBLP:conf/sigsoft/Gong023, DBLP:conf/icse/HaZ19, DBLP:conf/sc/MalikFP09, DBLP:conf/middleware/GrohmannNIKL19, DBLP:journals/corr/abs-2304-13032, DBLP:journals/pvldb/MarcusP19, DBLP:journals/tecs/TrajkovicKHZ22, DBLP:conf/splc/Acher0LBJKBP22, DBLP:conf/esem/ShuS0X20}. However, it is worth noting that most of these techniques are option selection methods as the configuration options often have redundant information and most of them have little influence on the software performance. Yet,~\citeauthor{DBLP:conf/sigsoft/Gong023}\cite{DBLP:conf/sigsoft/Gong023} discover that except for feature/option sparsity, which has been realized by most studies, the distribution of samples in the configuration landscape is also sparse---a significant property in the configuration performance learning problem that is worth further investigating.
    \item Section~\ref{sec:rq2.2} shows that the very basic version of DNN, i.e., MLP is the most commonly used learning model being employed by a total of 54 studies. This is evidence that a simple deep learning model is useful for learning software configurations and performance. This derives the exploitation of more complex DNN, for example, rDNN~\cite{DBLP:conf/icse/HaZ19, DBLP:conf/sigsoft/Gong023} is a DNN armed with regularization to address the problem of feature sparsity, and ResNet~\cite{DBLP:conf/wosp/CengizFAM23}---a type of neural network that incorporates residual connections to overcome the challenges of vanishing gradient for configurations embed into high dimensional representation. This demonstrates the potential of the deep learning models by addressing specific challenges and sheds light on future studies on improving the existing models.
    \item With the complicated architectures of deep learning models, one challenge for hyperparameter tuning is the explosion of search space. As such, we are pleased to reveal that 33 primary studies have addressed this challenge by exploring different heuristic methods to guide the tuning of hyperparameters while training deep learning performance models. For instance,~\citet{DBLP:conf/splc/GhamiziCPT19} employ the idea of natural selection and evolution to find the best population of hyperparameter configurations, which is robust to noise and outliers as the overall fitness is based on the collective behavior of the population rather than individual solutions. This diverse range of heuristic methods reflects the researchers' efforts to explore different approaches for optimizing hyperparameters and enhancing model performance, which should be kept by future researchers.
    \item In configuration performance learning tasks, the best optimization method for reducing the loss in training differs depending on the systems and performance attribute. For example, tasks with sparse features may benefit from adaptive optimization methods like Adam, while SGD is often used in situations where computational resources are limited. Thus, given that the relationship between configurations and performance of highly configurable software is often sparse, it is encouraging to find that 24 studies address this problem by leveraging Adam optimizer.
    \item Similarly, choosing the appropriate activation function can impact the DL model's performance, e.g., ReLU is effective in capturing complex, non-linear relationships. Hence, it is a promising behavior to see that ReLu is used in 30 primary studies to handle the non-linearity specializing the problem of configuration performance prediction.
\end{itemize}

Conversely, we have identified the following bad smells:
\begin{itemize}
    \item Given that sparsity has been addressed by 52 out of 85 papers, 24 of them rely on human efforts to select the correct feature sets to reduce sparsity, which is of low efficiency and low generalizability. In addition, there are still 33 works that did not acknowledge the sparsity issue. Moreover, only one study focused on solving the sparsity problem from the perspective of sample distributions~\cite{DBLP:conf/sigsoft/Gong023}, which could be a key aspect of future research. 
    \item Recall from Section~\ref{sec:rq2.2}, there are 55\% studies (47 out of 85) that provide no justification for their choices of deep learning models, which is a concern. It is essential for researchers to clarify their reasons for selecting specific models, as this enhances the understanding of the research motivations and contributions~\cite{DBLP:journals/tosem/LiuGXLGY22}. In the meantime, the lack of explicit explanations of model selection could be harmful to the community as researchers may miss out on important considerations or potential limitations.
    \item A great portion (52 out of 85) of papers choose to tune the hyperparameters manually, which is time-consuming and not generalizable. Besides, a subset of six studies relies solely on default hyperparameters that may not be optimal for all scenarios. This limitation may restrict the exploration of the optimal hyperparameter settings and hinder the potential of deep learning models~\cite{DBLP:journals/csur/YangXLG22, DBLP:conf/sc2/FrankHLB17}. As such, it is important for researchers to consider automatic tuning methods in order to maximize the performance and robustness of deep learning models. 
    \item Surprisingly, more than half of the studies (46 out of 85) omitted information on their choices of optimization and activation approaches. This omission poses a significant challenge to understanding and reproducing the deep learning models' results and findings~\cite{DBLP:conf/msr/GongC22, DBLP:conf/icse/HaZ19, DBLP:conf/sigsoft/Gong023}. Therefore, justification for these decisions should be provided in future works, as it allows practitioners to comprehend the rationale behind the decision-making. 
\end{itemize}









\subsection{Evaluation} 

Several noticeable common practices can be observed in the evaluation aspect of deep configuration performance learning from Section~\ref{sec:rq3}. Notably, the positive behaviors encompass:
\begin{itemize}
    \item A variety of metrics for accuracy has been applied is a rather positive sign for the community, as \citeauthor{mathews1994towards}~\cite{mathews1994towards} point out, no single measure gives an unambiguous indication of the modeling performance. More importantly, we have discovered that all the primary studies have leveraged some form of repeated evaluation procedure. This is crucial to ensure that the results were not produced due to chance or biased samples.
    \item Almost all studies have conducted comparisons between their models with existing works, and a few of them have utilized statistical tests and effect size tests to ensure the statistical significance and effect size difference of the comparison. This practice is vital in deep learning research as it enhances the reliability and robustness of the findings.
    \item Another positive observation is that 48 studies have considered multiple subject systems in their experiments. This is significant because evaluating the proposed model on software from different domains, scales, and performance indicators demonstrates its generalizability and robustness~\cite{ DBLP:conf/icccnt/KumarMBCA20, DBLP:conf/noms/SanzEJ22, DBLP:conf/bigdataconf/GhoshalWPS19, icse2020-empirical, DBLP:conf/icse/HaZ19}.
    \item Moreover, it is encouraging to see that the primary studies have examined a variety of domains. This diversity in domain coverage enhances the credibility and applicability of the findings across various contexts, providing broader insights for developers and practitioners.
\end{itemize}

On the contrary, the bad smells consist of:
\begin{itemize}
    \item We found that MAPE is the most widely used metric, due primarily to the fact that it is unit-free and easy to calculate. However, it is known that MAPE suffers the problem of being \emph{asymmetric} on the error above and below the actual value~\cite{goodwin1999asymmetry}, where the former receives a much greater penalty. As a result, such a strong bias tends to be problematic. 
    \item A notable concern arises from the fact that a significant majority of studies, around 93\% (79 out of 85), did not conduct any statistical tests, and 95\% of studies did not measure the effect size. This represents a significant problem as it introduces a potential source of randomness and uncertainty in the comparison results, limiting the ability to draw reliable conclusions and increasing the risk of causing severe external threats to validity. This highlights the need for greater awareness and adoption of statistical analysis in deep learning research. 
    \item It is worth noting that a significant proportion of studies (44\% of 85) evaluate their models on only one software, which can be considered a potential threat to the validity of the results and findings of the study. 
    Indeed, software systems of different characteristics can exhibit unique performance behavior due to factors such as architecture, complexity, and usage patterns. Therefore, it is important for future studies to evaluate their models on multiple software systems, spanning various domains, scales, and performance indicators, to ensure the robustness and learning ability of the proposed performance models. 
\end{itemize}
 



\subsection{Application} 

According to Section~\ref{sec:rq4}, applying the deep learning model to predict configuration performance is also subject to good practices and bad smells. Particularly, we confirm a few good practices:
\begin{itemize}
    \item The best practice in the model applications is their widespread adoption across various domains and for different tasks. This diversity is critical as it showcases the potential of performance models in addressing diverse challenges, and provides practical insights for researchers in different fields~\cite{DBLP:journals/jss/PereiraAMJBV21}.
    \item The most encouraging trend is that 29 out of 85 studies have actively considered multiple and dynamic environments, demonstrating the robustness of models. Acknowledging that software systems run under multiple and potentially varying environments is an important property as the behavior of software could be completely different across the environments~\cite{muhlbaueranalyzing,DBLP:conf/wcre/Chen22,DBLP:conf/wosp/PereiraA0J20}. By accounting for dynamic workloads, versions, and hardware in real-world scenarios, these studies contribute to a more comprehensive understanding of how performance models can be applied in practical settings.
    \item 19 out of the total studies have embraced the principles of open science by providing a public repository that includes source codes and datasets. This is a good practice as it allows researchers to replicate or reproduce the experiment results, build further research based on the existing knowledge, and collaborate with each other~\cite{DBLP:journals/tosem/LiuGXLGY22}.
\end{itemize}

Meanwhile, the negative smells encompass:
\begin{itemize}
    \item A potential concern is that 57 studies only consider pure prediction tasks, while these studies contribute valuable insights into performance prediction, it raises the question of whether these models can effectively be applied to other tasks beyond prediction, in other words, the applicability and generalizability of performance models across different domains and tasks remain unclear, especially when the usefulness of the model is merely measured by accuracy metrics.
    \item Another bad smell is that 66\% of 85 primary studies have solely focused on datasets from a single environment without considering dynamic factors that can impact model performance, which means there is a risk of overestimating the model's capabilities or encountering unexpected issues when applied in real-world scenarios~\cite{muhlbaueranalyzing}. Therefore, it is essential for future research to address this limitation by actively incorporating dynamic environments into their evaluation processes.
    \item It is concerning to note that a significant number of studies (78\%) still missed the opportunity to promote open science by not providing public repositories. This is a limitation as it restricts the replicability, reproducibility, and development of the community, which could be addressed by future studies. Further, among the 19 studies that offer an open-access repository, only 14 of them provide both source codes and datasets. 
    %\item Notably, although~\citet{DBLP:journals/tnse/CaoPC22} present a link in their paper, the link has already expired, and the repository is unavailable, which is rather a problematic practice. Therefore, it is essential for authors to maintain the accessibility of their repositories.
\end{itemize}






==> standalone.tex <==
% \documentclass[a4paper,10pt]{article}
% \usepackage{adjustbox}
% \usepackage{booktabs}
% \usepackage{csquotes}
% \usepackage{geometry}
% \usepackage{multirow}
% \usepackage[figuresright]{rotating}
% \DeclareMathAlphabet\mathbfcal{OMS}{cmsy}{b}{n}


% % \geometry{
% % left=3cm, % Adjust the left margin
% % right=3cm,  % Adjust the right margin
% % top=1cm,  % Adjust the top margin
% % bottom=1cm  % Adjust the bottom margin
% % }

% \begin{document}









% \begin{table}[t!]
% \centering
% \footnotesize
% \caption{SMBO models.}


% \begin{adjustbox}{width=\linewidth,center}

% \begin{tabular}{llllp{5cm}} 
% \toprule
% \textbf{SMBO model} & \textbf{Feature selection} & \textbf{Surrogate model} & \textbf{Acfunc} & \textbf{Acfunc search method} \\ \hline
% \texttt{ResTune} & Pre-selection & GP & EI & Numerical optimization \\ \hline
% \texttt{RoboTune} & Random forest & GP & GP-Hedge & Numerical optimization \\ \hline
% \texttt{Tuneful} & Sensitivity analysis & GP & EI & Numerical optimization \\ \hline
% \texttt{ATConf} & \# & GP$_{dropout}$ & LCB & Numerical optimization \\ \hline
% \texttt{FLASH} & \# & CART & Value & All configuration \\ \hline
% \texttt{BOCA} & \# & RF & EI & Screened all configuration \\ \hline
% \texttt{SMAC} & \# & RF & EI & Random sample and exploration around good configuration \\ \hline
% \texttt{OtterTune} & Lasso & GP & LCB & Random sample and exploration around good configuration \\
% \\ \bottomrule

% \end{tabular}
% \end{adjustbox}
% \label{tb:SMBO}
% \end{table}






% \begin{sidewaystable}[t!]
% \centering
% \footnotesize
% \caption{Models.}

% \begin{adjustbox}{width=\linewidth,center}
% \begin{tabular}{lp{4cm}p{3cm}p{3cm}p{3cm}p{3cm}p{3cm}l}
% \toprule
% \textbf{Model} & \textbf{Description} & \textbf{Advantages} & \textbf{Disadvantages} & \textbf{Applicability} & \textbf{Hyperparameters} & \textbf{Used in SMBO} & \textbf{References} \\ \hline
% \texttt{SVR} & A model map data to a high-dimensional space, construct a linear regression model and employ kernel functions for non-linear regression. & Addressing high-dimensional problems & High sensitivity to parameter choice and kernel function; & General & Regularization parameter, kernel type, etc. & - & \cite{SVM} \\ \hline
% \texttt{LR} & A model assume a linear relationship between configurations and directly fit parameters. & Simple algorithm and fast execution & Only suitable for linear relationships. & General & None & - & - \\ \hline
% \texttt{GPR} & A classic Bayesian optimization model provide predictions and probability distributions. & Providing uncertainty estimates and high flexibility & Limited in high-dimensional datasets; Requires kernel function selection. & General & Length scale, signal variance etc. & atconf, ottertune, restune, robotune, tuneful & \cite{GPR} \\ \hline
% \texttt{DT} & A non-parametric model using tree structures for feature segmentation. & Handling non-linear and complex relationships and easy interpretation & Overfitting and instability. & General & Tree depth, criterion, etc. & flash & flash \\ \hline
% \texttt{RF} & A machine learning mdoel integrating multiple decision trees. & Managing complex relationships, improving accuracy, and stability & Complexity and interpretability challenges. & General & Number of trees, depth, etc. & boca, smac & \cite{RF} \\ \hline
% \texttt{DECART} & A model Combine CART with resampling and parameter adjustment for performance prediction. & Handling non-linear and complex relationships & Overfitting & General & Number of trees, information computation metrics, etc. & - & \cite{SPL} \\ \hline
% \texttt{SPLConqueror} & A model learn individual configuration options and mutual influences from differences in sample measurements. & Efficiently handling complex relationships; & Computational cost is relatively high. & Highly Configurable Systems & Learning rate, sampling methods, etc. & - & \cite{DECART} \\ \hline
% \texttt{DeepPerf} & A model combine DNNs with sparse regularization techniques to automatically adjust network hyperparameters. & High accuracy for binary and/or numeric configurations; & High data requirements and black-box nature. & Highly Configurable Systems & Network layers, regularization parameters, etc. & - & \cite{DeepPerf} \\ \hline
% \texttt{DaL} & A model divide configuration samples into different parts and build a separate DNN model for each part. & Efficiently addressing feature sparsity & High data requirements and black-box nature. & Highly Configurable Systems & Number of partitions, DNN structure, etc. & - & \cite{DaL} \\ \hline
% \texttt{HINNPerf} & A Hierarchical interactive neural network use embedding methods and layered network blocks to model complex interactions between configuration options. & Enhanced accuracy through hierarchical modeling & High data requirements and black-box nature. & Highly Configurable Systems & Embedding dimensions, hierarchical regularization parameters, etc. & - & \cite{HINNPerf} \\ \hline
% \texttt{Perf-AL} & A DNN combine adversarial learning with generative networks and regularization techniques. & High accuracy with minimal training samples & High data requirements and black-box nature. & Highly Configurable Systems & Adversarial parameters, training iterations, etc. & - & \cite{PerfAL}
% \\ \bottomrule

% \end{tabular}
% \end{adjustbox}
% \label{tb:models}
% \end{sidewaystable}









% \begin{table}[t!]
% \centering
% \footnotesize
% \caption{Datasets.}


% \begin{adjustbox}{width=\linewidth,center}

% \begin{tabular}{lllllllll}
% \toprule
% \textbf{Dataset} & \textbf{Domain} & \textbf{$|\mathbfcal{B}|$/$|\mathbfcal{N}|$} & \textbf{$|\mathbfcal{C}|$} & \textbf{Budget} & \textbf{$\mathbfcal{S}_{train}$} & \textbf{$\mathbfcal{S}_{space}$} & \textbf{Used by} \\ \hline
% \textsc{DeepArch} & Exploration tool & 12//0 & 4096 & 207 & 60 & 3.45E+41 & A design space \\ \hline
% \textsc{MariaDB} & Database & 8//3 & 972 & 226 & 192 & 5.31E+11 & About \\ \hline
% \textsc{MongoDB} & Database & 14//2 & 6840 & 278 & 392 & 3.14E+10 & About \\ \hline
% \textsc{Lrzip} & File Compressor & 11//0 & 191 & 184 & 55 & 393216 & Analyzing \\ \hline
% \textsc{DConvert} & Image Scaling & 17//1 & 6764 & 335 & 578 & 10485760 & Analyzing \\ \hline
% \textsc{SQLite} & Database & 14//0 & 1001 & 299 & 70 & 16384 & BEETLE \\ \hline
% \textsc{storm} & Data analytics & 0//12 & 1557 & 263 & 288 & 2.83E+23 & BEETLE \\ \hline
% \textsc{Hadoop} & Data analytics & 2/7 & 3994 & 297 & 192 & 1.27E+29 & CM-CASL \\ \hline
% \textsc{redis} & Database & 1//8 & 4400 & 298 & 192 & 5.78E+16 & CM-CASL \\ \hline
% \textsc{tomcat} & Web Server & 0//12 & 3600 & 282 & 288 & 7.93E+34 & CM-CASL \\ \hline
% \textsc{spark} & Data analytics & 5//8 & 2700 & 326 & 200 & 2.55E+12 & CM-CASL \\ \hline
% \textsc{Apache} & Web Server & 8//0 & 192 & 133 & 40 & 256 & DeepPerf \\ \hline
% \textsc{LLVM} & Image Processing & 10/0 & 1024 & 182 & 50 & 2048 & DeepPerf \\ \hline
% \textsc{BDBC} & Video Encoder & 16//0 & 2560 & 259 & 80 & 46080 & DeepPerf \\ \hline
% \textsc{HSMGP} & Database & 11//3 & 3456 & 218 & 363 & 297271296 & DeepPerf \\ \hline
% \textsc{BDBJ} & Database & 31//2 & 13485 & 371 & 1008 & 3.30E+12 & DeepPerf \\ \hline
% \textsc{JavaGC} & Multi-Grid Solver & 12//23 & 166975 & 289 & 1922 & 2.67E+41 & DeepPerf \\ \hline
% \textsc{SQLite} & Database & 39//0 & 4553 & 206 & 195 & 5.50E+11 & DeepPerf \\ \hline
% \textsc{sort-256} & Database & 0//3 & 206 & 127 & 48 & 2016 & flash \\ \hline
% \textsc{wc-c4-3d} & Data analytics & 0//3 & 756 & 230 & 48 & 849999150 & flash \\ \hline
% \textsc{noc-CM-log} & Database & 1//3 & 259 & 129 & 55 & 2376 & flash \\ \hline
% \textsc{SaC} & Compiler & 52//7 & 65424 & 316 & 2704 & 3.14E+28 & flash \\ \hline
% \textsc{polly} & Code optimizer & 39//0 & 60000 & 285 & 195 & 2$^{39}$ & HINNPERF \\ \hline
% \textsc{vp9} & Video Encoder & 41//0 & 216000 & 271 & 205 & 2$^{41}$ & HINNPERF \\ \hline
% \textsc{Brotli} & File Compressor & 1//2 & 2160 & 203 & 55 & 308 & Twins \\ \hline
% \textsc{HSQLDB} & Database & 18//0 & 864 & 149 & 90 & 262144 & Twins \\ \hline
% \textsc{PostgreSQL} & Database & 6/3 & 19008 & 298 & 108 & 1415577600 & Twins \\ \hline
% \textsc{xgboost} & Model Tuning Tool & 11//0 & 2048 & 278 & 55 & 1.50E+10 & Twins \\ \hline
% \textsc{ExaStencils} & Code Generator & 7//5 & 86058 & 416 & 224 & 1610612736 & Twins \\ \hline
% \textsc{7z} & File Compressor & 11//3 & 68640 & 382 & 363 & 167772160 & Twins \\ \hline
% \textsc{Apache} & Web Server & 14//2 & 13440 & 271 & 392 & 234881024 & Twins \\ \hline
% \textsc{kanzi} & File Compressor & 31//0 & 3202 & 237 & 160 & 2147483648 & Twins \\ \hline
% \textsc{jump3r} & Audio Encoder & 37//0 & 4297 & 232 & 185 & 204472320 & Twins
% \\ \bottomrule

% \end{tabular}
% \end{adjustbox}
% \label{tb:dataset}
% \end{table}




% % \bibliographystyle{plain}
% % \bibliography{references}
% \end{document}
